Transaction Propagation on Permissionless Blockchains: Incentive and Routing Mechanisms

Existing permissionless blockchain solutions rely on peer-to-peer propagation mechanisms, where nodes in a network transfer transaction they received to their neighbors. Unfortunately, there is no explicit incentive for such transaction propagation. Therefore, existing propagation mechanisms will not be sustainable in a fully decentralized blockchain with rational nodes. In this work, we formally define the problem of incentivizing nodes for transaction propagation. We propose an incentive mechanism where each node involved in the propagation of a transaction receives a share of the transaction fee. We also show that our proposal is Sybil-proof. Furthermore, we combine the incentive mechanism with smart routing to reduce the communication and storage costs at the same time. The proposed routing mechanism reduces the redundant transaction propagation from the size of the network to a factor of average shortest path length. The routing mechanism is built upon a specific type of consensus protocol where the round leader who creates the transaction block is known in advance. Note that our routing mechanism is a generic one and can be adopted independently from the incentive mechanism.

==> tex/Appendices.tex <==
\appendix
\section{Impossibility Result for 1-Connected Networks - Eclipse Attacks}\label{sec:appendix}

In 1-connected networks, there are critical nodes which have special positions in the propagation paths between some node pairs. 
A critical node for a node pair appears in all possible paths between these two nodes. 
The following lemma shows that non-competing advantage of critical nodes makes it impossible to have a Sybil-proof incentive mechanism for 1-connected networks.

\begin{lemma}[Impossibility Lemma]
In order to deviate nodes from introducing Sybil nodes in 1-connected networks, processing fee should be shared between the first propagating node and the round leader.
\end{lemma}
\begin{proof}
Assume that, because of 1-connectedness of the network, a node $n$ may have a critical position for a transaction $T$, meaning that it is certain that he will be included in the propagation path of that transaction.

\begin{figure}
	\begin{center}
\includegraphics[scale=0.5]{figures/sybil_appendix.pdf}
\caption{The fee sharing before and after a Sybil node $n_{i'}$ added by $n_i$}\label{fig:sybil_appendix}
\end{center}
\end{figure}

Now, we investigate the share of a node $n_i$ with and without a Sybil node. 
As seen in Figure \ref{fig:sybil_appendix}, $n_i$ is the $i^{th}$ node in the propagation path and his corresponding fee shares are $\f{k}{i}$ and $\f{k+1}{i} +\f{k+1}{i+1}$. 
In order to demotivate $n_i$, $\f{k}{i}$ should be greater than or equal to $\f{k+1}{i} +\f{k+1}{i+1}$.  
Since the position of node would change for different transactions and rounds, the condition should hold for all positions:
\begin{eqnarray*}%{rll}
	\forall\, i \in \{1,\ldots, k\}, \quad &&\f{k}{i} \geq \f{k+1}{i} + \f{k+1}{i+1} \\
	\text{(summing for all $i$'s)}\implies &&\sum_{i=1}^{k} \f{k}{i} \geq \sum_{i=1}^{k} \f{k+1}{i} + \sum_{i=1}^{k} \f{k+1}{i+1} \\
	\text{(Definition of $\mathcal{F}$)}\implies && \ff \geq \ff - \f{k+1}{k+1} + \ff - \f{k+1}{1} \\
	\implies &&\f{k+1}{k+1} +  \f{k+1}{1} \geq \ff \\
	\text{(Definition of $\mathcal{F}$)} \implies &&\f{k+1}{k+1} +  \f{k+1}{1} = \ff \,.
\end{eqnarray*}
Therefore, there will not be any incentive for the rest to propagate $T$ which contradicts with rational behavior. 
\end{proof}


%The only possible way to make this scheme work is that each node should act like the client so that they can not be sure the transaction coming from either client or some intermediary node.
%In other words, we show that generic incentive function, that works in any network assumptions and motivates all propagating nodes, is not possible.

%\section{Fee Sharing for Bitcoin-NG-like Schemes}\label{sec:appendix2}
%%\todo{Bitcoin-NG requires additional analysis since the leaders share is 40\% for current, 60\% from previous one.}
%For some consensus protocols, transactions fees are shared among the leaders of different round leaders.
%In this manner, we first show that the share of the other round leaders cannot be arranged from the share of the current round under the assumptions derived in Section \ref{sec:incentive}.
%\begin{lemma}
%It is not possible to deduct shares of other rounds leaders from the share of current round leader.
%\end{lemma}
%\begin{proof}
%Here, all conditions (\ref{eqn:infunc_1}), (\ref{eqn:infunc_2}) and (\ref{eqn:infunc_3}) given in Section \ref{sec:incentive} holds. However, the fundamental assumption $\sum_{i=1}^{k}\f{k}{i}=f$ is changed to $\sum_{i=1}^{k-1}\f{k}{i}+\alpha \f{k}{k}=f$ where $\alpha>1$ is the coefficient regarding shares of other round leaders, e.g., in Bitcoin-NG, $\alpha=2.5$. We can see that for any $\alpha$ and $C$ value restricts $k$ value.
%\begin{eqnarray*}
%\text{Using (\ref{eqn:infunc_1})} &\quad &\sum_{i=1}^{k} \f{i}{i} \geq \sum_{i=1}^{k} \f{i+1}{i+1} + \sum_{i=1}^{k} \f{i+1}{i}\\
%\text{Using (\ref{eqn:infunc_3})} &\implies& \alpha^{-1}f=\f{1}{1} \geq \f{k+1}{k+1}+ \sum_{i=1}^{k} \f{i+1}{i} \\
%&& \geq \f{k+1}{k+1}+ \sum_{i=1}^{k} \f{k+1}{i}   = f - (\alpha-1)\f{k+1}{k+1} \\
%\text{Using (\ref{eqn:infunc_2})} &\implies& \f{k+1}{k+1} \geq \alpha^{-1} f \implies \f{i}{k}=\f{i}{i+1} \geq C \cdot \alpha^{-1} f \\
%&\implies& (\forall k),\, f = \sum_{i=1}^{k-1}\f{k}{i}+\alpha \f{k}{k} \geq (k+\alpha-1)C \cdot \alpha^{-1} f \\
%&\implies& (\forall k),\,\alpha \geq C (k+\alpha-1)  \implies \alpha C^{-1} +1 - \alpha \geq k  \Rightarrow\!\Leftarrow
%\end{eqnarray*}
%\end{proof}
%
%
%On the other hand, the equation can be changed to $\sum_{i=1}^{k}\f{k}{i}=\beta f$, i.e., the share can be deducted from the total ($\beta=2/5$ in Bitcoin-NG).
%Since analyses of the fee sharing function is independent of $f$ value, we can assume $f'=\beta f$ and verify the same conditions.

%\section{Experimental Results for Routing Mechanism}\label{sec:appendix3}

%\begin{table}
%	\caption{Experimental results for different network and connection sizes. AVP: Average Path Length, ANVN: Average Number of Visited Nodes per transaction, BW Gain: Bandwidth Gain percentage compared to conventional broadcasting}
%	\begin{tabular}{|c|c|c|c|c|c|c|c|}
%		\hline 
%		G(N,m) & G(50,4) & G(50,8) & G(100,4) & G(100,8) & G(500,4) & G(500,8) & G(500,16) \\ 
%		\hline 
%		APL & 1.50 & 1.50 & 2.04 & 1.86 & 2.74 & 2.45 & 2.09  \\ 
%		\hline 
%		ANVN & 4 & 8 & 6 & 10.98 & 8 & 13.98 & 25.01  \\ 
%		\hline 
%		BW Gain &   &  &   &   &  &  &  \\ 
%		\hline 
%		\hline 
%		G(N,m) & G(1000,4) & G(1000,8) & G(1000,16)  &  G(2000,8) & G(2000,16) & G(5000,8) &G(5000,16)\\ 
%		\hline 
%		APL & 2.97 & 2.65 & 2.30 & 2.81 & 2.50 & 3.03 & 2.72 \\ 
%		\hline 
%		ANVN & 9.05 & 15.17 & 27  & 16.78 & 28.97 & 17.96 & 31.77 \\ 
%		\hline 
%		BW Gain  &  &  &  &  &  &  & \\ 
%		\hline 
%	\end{tabular}
%\end{table}
%
%\begin{table}
%	\caption{Experimental results for the probability of a transaction cannot reach to the round leader in the presence of $f\%$ of nodes failing during the transaction phase}
%	\begin{tabular}{|c|c|c|c|c|c|c|c|}
%		\hline 
%		G(N,m) & G(50,4) & G(50,8) & G(100,4) & G(100,8) & G(500,4) & G(500,8) & G(500,16) \\ 
%		\hline 
%		$f=0.2$ & 0.04 & 0 & 1.56 & 0.02 & 8.06 & 0.27  & 0  \\ 
%		\hline 
%		$f=0.3$  & 0.12 & 0 & 5.91 & 0.11 & 11.19 & 1.08 & 0  \\ 
%		\hline 
%		$f=0.4$  &  0.19 & 0.01 & 9.68 & 0.98 & 30.02 & 5.21 & 0.19 \\ 
%		\hline 
%		\hline 
%		G(N,m) & G(1000,4) & G(1000,8) & G(1000,16)  &  G(2000,8) & G(2000,16) & G(5000,8) &G(5000,16)\\ 
%		\hline 
%		$f=0.2$  & 9.88 & 0.53 & 0 & 1.41 & 0 & 1.75 & 0\\ 
%		\hline 
%		$f=0.3$  & 16.88 & 2.12 & 0.02  & 3.14 & 0.05 & 8.09 & 0.06 \\ 
%		\hline 
%		$f=0.4$   & 34.79 & 7.57 & 0.85 & 11.38 & 0.36 & 12.34 & 1.02\\ 
%		\hline 
%	\end{tabular}
%\end{table}


==> tex/Introduction.tex <==
\section{Introduction}

After acknowledgment of Bitcoin \cite{nakamoto2008bitcoin} as a digital cryptocurrency, blockchain has become a trending subject to not only the research community but also the industrial society because of the enormous application area. 
The blockchain can be defined as a decentralized immutable public ledger which is updated and secured in a distributed structure among the untrusted parties.
This ledger consists of ordered blocks, which may be composed of transactions like in Bitcoin or smart contracts as in Ethereum \cite{wood2014ethereum}.

There are a variety of blockchain types trying to achieve decentralization and immutability in different settings.
Main distinguishing characteristics are the access structure and the consensus protocol.
%Blockchains differ with respect to the answers to the following questions:
%who is eligible to contribute to the ledger? How they validate the ledger?
Consensus protocols are used to validate the ledger and to maintain consistency in the ledgers stored individually. 
Regarding the authorization, there are two types of blockchains: 
permissionless where anyone can join and contribute to the chain, and permissioned which requires an authorization to join the network.
%permissionless (public) and permissioned.
%In permissionless blockchain, anyone can join to the network and contribute without an authorization. 
%Permissioned blockchain, conversely, has an authority deciding who can contribute to the ledger. 
%In general, consensus on a chain can be achieved by either a consortium (e.g. Byzantine agreement \cite{byzantine}) among (subset of) all participants or the implicit validation of the legitimate blocks (e.g. Bitcoin).
%We differ explicit and implicit in a way that, in former one, each participant provides a proof which is an evidence on his consult for the block whereas, in the latter one, participants show their consult by working on the same chain.
%In any case, all information is advertised to the round leader(s), whose identity may not be available, after the validation it is included to the block and broadcast.
%\textbf{Permissionless blockchain.}
Authorization of the blockchain influences the other components of the blockchain as well. 
Since permissionless blockchains consist of anonymous or pseudonymous users, they require Sybil-proof consensus protocol and incentive-compatible participation \cite{peters2016understanding}.
First, in order to prevent Sybil attacks, participation or validation in a permissionless blockchain should require proof-of-something that cannot be fabricated like mining work \cite{nakamoto2008bitcoin}, possession of stake \cite{king2012ppcoin} or storage of data \cite{dziembowski2015proofs}. 
Second, participation in each process of the blockchain should comply with the rational behavior where participants try to maximize their revenue \cite{peters2016understanding}.
%There should be an incentive for each operation requiring communication or computational cost.

%Among several advantages of blockchain technology, there are issues regarding the propagation of information needed to be addressed. 
%In addition, transmission is controlled by the central authority and may not require an incentive for transferring information.

\textbf{Rationalism.} 
There is no surprise that transition from a centralized system into distributed one brings along game theoretical concerns \cite{monderer1999distributed}. 
%Indeed, rational behavior of the users has been observed in peer-to-peer networks \cite{adar2000free,huberman1997social,Shneidman2003}.
Importance of the game theoretical analysis in blockchain technology is already demonstrated by the selfish mining attack \cite{eyal2014majority,nayak2016stubborn,sapirshtein2016optimal}.
Recently, Rational Protocol Design framework has been introduced and applied on Bitcoin to analyze incentives for the miners \cite{Garay:2013:RPD:2570450.2570634,eurocrypt18rational}. 
These incentive analyses are not limited to mining operation.
In a permissionless blockchains where each rational node trying to maximize its revenue,
each operation requires an incentive for participation \cite{peters2016understanding}.
Information propagation mechanism, as one of the essential operations, should be incentive compatible.
%Though they mainly focused on the security model of the blockchain, these analyses are also important for a sustainable system \cite{peters2016understanding}.
%In the long term, altruistic behavior is not sustainable for the permissionless blockchains, especially for cryptocurrencies \cite{kaskaloglu2014near,kroll2013economics}. 
%Incentive concern is mainly addressed for the validation of the transactions.
%Existing blockchain solutions, including Bitcoin and Ethereum, reward only the one who validates the transactions, not the ones who propagate them.
%Yet, the incentive for the propagation of these transactions is altruistically fulfilled \cite{altruism}.
%Especially for the permissionless blockchains, information propagation should be incentive-compatible just like any other non-free operation.

%\textbf{Existing applications.} 
The aforementioned problem seems to be underrated and mostly ignored since the most successful permissionless blockchain applications, including Bitcoin and Ethereum, work without any direct incentive to propagate. 
If we continue with the Bitcoin example, there are two consecutive reasons for that: altruism, and centralized mining.
Bitcoin is evolved from altruistic participation into centralized mining pools.
Early adopters were enthusiastic and contributed to information propagation altruistically \cite{altruism}.
At the moment, conversely, the environment turned into a rational but centralized system where only a few number of pools control the network \cite{kroll2013economics,gervais2014bitcoin,miller2015discovering,gencer2018decentralization}.
In the current setting, a client who wants to advertise a transaction needs to reach a node of the pool, instead of all miners in that pool. %then internal propagation is controlled by the pool.
Consequently, the existing applications do not exhibit fully decentralized blockchain properties and do not conflict with the necessity of the incentive.

The incentive of the propagation is also relevant to the bounty on the transaction, namely transaction fee. 
Each transaction has a specific transaction fee which can be zero. %, and there are block rewards which are given to the miner independently from the transactions included in that block.
%The one who mines the block earns both the block reward and fees of the included transactions.
Transaction fees encourage the miners to validate and add them to the block.
There is no incentive to validate transactions with zero transaction fees \cite{kaskaloglu2014near}. 
Knowledge of a transaction is as precious as its transaction fee.
The more it is known by the network, the less probability that a specific node has a chance to profit from its fee. 
For that reason, a rational node has an incentive \textbf{not} to propagate the incoming transaction knowledge with the rest of the network. 
Contradictorily, the more a client pays a transaction fee, the less rational nodes are willing to propagate, thereby the later it is expected to be validated.
The same problem holds for all permissionless blockchains supposed to work in a rational participation assumption.

%Lack of incentive in information propagation in the peer-to-peer networks has been studied in the last decades \cite{drucker2012simpler,emek2011mechanisms,kleinberg2005query,li2009incentive}. 
%The proposed solutions are not applicable for the permissionless blockchains.
%In peer-to-peer solutions, participants are asked to provide a specific datum like the position of a peer or the answer to a query.
%In blockchains, it is requested to validate the transactions and place them into a valid block.
%In the latter case, participants can always compete for the reward without propagating, whereas in the former one, peers who have the datum do not need to propagate anymore and the others must propagate to have a chance.
%Recently, blockchain oriented propagation mechanisms have been proposed \cite{abraham2016solidus,babaioff2012bitcoin}.
%Babaioff et al. \cite{babaioff2012bitcoin} presented the lack of incentive to propagate transactions in the Bitcoin, and they provided a solution for the $d$-ary directed tree networks. 
%In \cite{abraham2016solidus}, the authors investigate the propagation of not only the transaction but also the block itself.

%There have been several proposals on content sharing and streaming applications \cite{vishnumurthy2003karma,sirivianos2007dandelion,ngan2004incentives,CPE:CPE1189}.

\textbf{Routing.} 
Existing propagation mechanisms suffer from the ineffective routing of the information from a source (client) to the destinations (miners).
In a centralized system, propagation can be handled very efficiently by a predefined routing mechanism because the location of the server is known and stable.
%For instance, in a network with millions of participants, direct routing would reduce the cost from the order of millions to order of tens.
%This comes from the small world phenomenon \cite{travers1967small}, which states that the distance between any two nodes is extremely small regarding the network size.
The dynamic and decentralized structure of blockchain prevents from having stationary efficient propagation routes.

It is reasonable and necessary to broadcast all validated information through the network since the public ledger is stored and validated by all contributing nodes. 
In the existing blockchains, there is additional broadcasting of the information before being validated.
At first, every information is propagated throughout the network, then a node (miner) validates it and after validation, it is again propagated within the block.
Even more redundancy is caused by the flooding of each information because a node will receive the same information from different neighboring nodes.
This additional cost is already reduced by sending the digest of the information to check whether the neighbor has it or not.
If the size of the information is relative to hash, then the cost of a broadcasting would be significantly more than double of the network size.
Statoshi info \cite{statoshi}, a block explorer of Bitcoin, shows that average incoming bandwidth usage for the transactions (\texttt{tx}) is $2.87$ KBps, whereas for the checking messages (\texttt{inv}) is $4.12$ KBps (measurements taken between 02:00 AM and 14:00 PM in 13 of Feb. 2018).

For some consensus protocols as in Bitcoin, the redundancy is inevitable because of the unpredictability of the node (round leader) who will create the new block. 
This is caused by the fact that the block owner is simultaneously validated with his proposed block. 
Nevertheless, there have been recent proposals where the legitimate block owner can be validated before the block is proposed \cite{abraham2016solidus,bentov2016cryptocurrencies,bentov2014proof,eyal16bitcoin,ouroboros}, which we call \textit{first-leader-then-block} consensus protocols.
In a first-leader-then-block structure, it is possible to overcome redundant communication cost by routing information from a client to the round leader.

\subsection{Our Contributions}

In this work, we investigate two information propagation related problems of block\-chains: incentive and bandwidth efficiency. 
We present a generic incentive mechanism for information propagation, a routing mechanism compatible with first-leader-then-block consensus protocols and finally we combine them together in an efficient way.

Firstly, we formulate the ideal incentive function allocating the reward among the propagating participants for generic network model.
%We show the impossibility result of the Sybil-proofness for the 1-connected networks.
%2-connected network means that there are multiple paths between any two nodes in the network. 
%Nonetheless, we also show the impossibility result for 1-connected networks in Appendix \ref{sec:appendix}.
%For 2- or more connected graphs, we analyze the necessary and sufficient conditions to propagate a transaction as well as deviate participants from introducing Sybil nodes.
In this manner, we obtain the following results:
\begin{itemize}
	\item \textit{Impossibility}: In 1-connected networks, it is not possible to design Sybil-proof fee sharing function which allocates the fee among all the contributors.
	\item \textit{Equity}: Propagation decision of a node is independent of the neighbors' capacities. A rational node would propagate to either all of its neighbors or none of them.
	\item \textit{Rationality:} Each rational node having a probability less than $C$ for being the round leader (among the ones having the transaction) will propagate the transaction given the following formula:
	\begin{IEEEeqnarray*}{ll}
		\f{k}{i}= \begin{cases}
			\ff\cdot C(1-C)^{i-1} &\text{ for } i<k, \\
			\ff\cdot (1-C)^{k-1} &\text{ for } i=k,
		\end{cases}
	\end{IEEEeqnarray*}
	where $\ff$ is the total processing fee of the transaction, $k$ is the length of the propagation path from a client to the round leader, and $\f{k}{i}$ is the share of the $i^{th}$ node in that path.
\end{itemize}

Secondly, we present a routing mechanism which reduces the communication cost of the information propagation from the size of the network to the scale of average shortest path length.
It corresponds to a logarithmic scale of the network size for the random network models.
This mechanism is compatible with all blockchains where the round leader can be verified before the block is announced. 
In addition, we analyze the failure probabilities of a transaction to reach the round leader in the presence of the node who may fail or censor.
%The routing mechanism enjoys bandwidth efficiency while keeping the same security level against the location related attacks to the round leader.

Finally, we present an effective message propagation protocol which combines our incentive and routing mechanisms in a storage-efficient way.

The rest of the paper is organized as follows: 
Section \ref{sec:relatedwork} presents the related work.
Our blockchain model and notations are defined in Section \ref{sec:notation}.
Section \ref{sec:incentive} formulates requirements of the incentive problem and computes the generic solution. Smart routing mechanism is presented in Section \ref{sec:routing} and combined with incentive mechanism in Section \ref{sec:combined}. Finally, Section \ref{sec:conc} concludes the paper.



\section{Related Work}\label{sec:relatedwork}

The lack of information propagation incentive in a peer-to-peer network has been known and studied in different settings \cite{drucker2012simpler,emek2011mechanisms,kleinberg2005query,li2009incentive}. 
Kelinberg and Raghavan \cite{kleinberg2005query} proposed an incentive scheme for the answer to a query in a tree network model. 
Li et al. \cite{li2009incentive} focused on the peer discovery in a homogeneous network where each peer has the same probability to be a provider. 
Both systems try to locate a node (or a set of nodes) in the network, which has two main differences from the blockchain information propagation: participants do not compete against the ones who forwarded the message to them and participants cannot make up an answer for a query or location of a peer, i.e., either they have the right answer or not.
Whereas in the blockchain, every node is a leader candidate who can find the valid block which corresponds to the answer to a query.

In \cite{drucker2012simpler,emek2011mechanisms}, the authors analyzed the incentive problem for multi-level marketing which rewards referrals if their advertisement produces a purchase.
In these marketing models, the reward is shared among all participants in the tree including the propagation path.
Conversely, in our model, and \cite{abraham2016solidus,babaioff2012bitcoin} which are focused on the blockchain, it is shared between only the ones in the propagation path which is the direct path between the client and the leader.

The proposed solutions for peer-to-peer networks are not applicable for the permissionless blockchains.
In peer-to-peer solutions, participants are asked to provide a specific datum like the position of a peer or the answer to a query.
In blockchains, it is requested to validate the transactions and place them into a valid block.
In the latter case, participants can always compete for the reward without propagating, whereas in the former one, peers who have the datum do not need to propagate anymore and the others must propagate to have a chance.
Besides all, an important difference between message propagation in blockchain and the other peer-to-peer systems is that a blockchain participant has an incentive not to propagate the message whereas others do not since they cannot generate the required information by themselves.
Recently, blockchain oriented propagation mechanisms have been proposed \cite{abraham2016solidus,babaioff2012bitcoin}.
Babaioff et al. \cite{babaioff2012bitcoin} presented the lack of incentive to propagate transactions in the Bitcoin, and they provided a solution for the $d$-ary directed tree networks. 
In \cite{abraham2016solidus}, the authors investigate the propagation of not only the transaction but also the block itself.

In \cite{babaioff2012bitcoin}, Babaioff et al. uncovered the incentive problem in the Bitcoin system where a rational miner has no incentive to propagate a transaction. 
They focused on a specific type of network, namely regular $d$-ary directed tree with a height $H$, and assumed that participants have the same processing power.
In this setting, they presented an incentive scheme and proved that it is also Sybil-proof.
Abraham et al. recently proposed a consensus mechanism, Solidus, offering an incentive to propagate transactions and validated blocks (puzzles) \cite{abraham2016solidus}. 
In their proposal, the amount of processing fee passed to the next node is determined by the sender.
%, and they concluded to be a fixed amount at the end of their analysis.
%It requires detailed study on determining the charging amount since small value would not lead to propagation and high value may not have enough incentive for block owner. 
Both works adopted signature chaining mechanisms to prevent any manipulation over the path and thereby secure shares of each contributor.
Regarding the game theoretical analysis, former one \cite{babaioff2012bitcoin} assumes tree structure which eliminates competition for the common neighbors, whereas the latter one \cite{abraham2016solidus} analyzes only the case of competitions between nodes for shared neighbors.

To the best of our knowledge, there is no existing work on a direct routing mechanism for dynamic blockchain networks.
Nonetheless, Li et al. \cite{li2009incentive} presented a distributed routing scheme having the same structure as our solution.
The main difference is that they focused on one-to-one routing which is dedicated to a single target, whereas we do one-to-all, which connects the complete network to the round leader.
In addition, unlike \cite{li2009incentive}, we insert alternative routes as a precaution and analyze the failure probability of these temporary routes caused by momently failing nodes.
%Existing static networks solutions cannot be applied since the round leader who is responsible to gather the transactions is frequently changing.


\section{Our Blockchain Model and Notations}\label{sec:notation}
In this section, we present general characteristics of our blockchain model and our notation.
To keep it simple and consistent, in the rest of the paper, we will use the term transaction propagation, yet it can be replaced with any kind of information propagation.

\textbf{Access structure.} 
There are two types of blockchains: 
permissionless (public) and permissioned.
In permissionless blockchain, anyone can join the network and contribute without an authorization. 
Permissioned blockchain, conversely, has an authority deciding who can contribute to the ledger. 
%permissionless where anyone can join and contribute to the chain, and permissioned which requires an authorization to join the network.
Our work does not have a requirement in this manner, and we focus on the generic case: permissionless blockchain.

\textbf{Participants.}  
Since it is a permissionless blockchain, anyone can participate and contribute to the ledger directly.
Moreover, there is no discrimination between participants, i.e., they all have abilities to prepare a transaction as a client and to propose a block as a round leader. 
For identification, each participant has a public and private key pair and can be validated by his public key.

\textbf{Network.} 
It is a peer-to-peer network and each participant is matched with a node. 
%Each new node is, by default, connected to $N_{con}$ nodes in the network.
%Some nodes may decide to connect more nodes, default value will be used for simple estimations.
%The network is assumed to be a 2-connected graph, i.e., removal of any node would not disconnect the graph or there are multiple paths between any two nodes.

\textbf{Consensus and leader election.}
Incentive mechanism defined in Section \ref{sec:incentive} works regardless of the consensus structure. 
Whereas, the routing mechanism requires special treatment, which we called \textit{first-leader-then-block} consensus protocols.
First-leader-then-block (\textit{FLTB}) protocols can be defined as the consensus model where the round leader is validated before he proposes the block.
Any leader election mechanism which is independent of the non-validated transactions can be converted into \textit{FLTB} type.
Examples of the \textit{FLTB}-based blockchains are Bitcoin-NG \cite{eyal16bitcoin} and several PoS-based ones  \cite{abraham2016solidus,bentov2016cryptocurrencies,bentov2014proof,ouroboros}.

%Furthermore, there could be multiple round leaders at a round, both mechanisms can be applied in these scenarios. 
% the routing mechanism will still be efficient as long as the leader set compose a relatively small subset of the participants.

The rest of the definitions and notations are listed below:
\begin{itemize}
	\item \textit{Node}: A participant of the blockchain in the network. We may use the terms node and participant interchangeably. 
	\item \textit{Neighboring}: Direct connection in the network, adjacency in the graph.
	\item \textit{Client}: The source or the sender of a transaction. Client of a transaction $T$, denoted by $c_T$. %Note that client could be a miner at the same time.
	\item \textit{Round Leader}: The legitimate participant responsible to construct the block. 
	%For simplicity, we will assume there is only one leader, but our mechanisms can be applied for systems having multiple leaders at the same time. %As long as the number of leaders is not proportional to the network size, it will be significantly bandwidth-efficient.
	\item \textit{Intermediary Node}: A node on the transmission path between the round leader and a client.
	\item $\mathcal{L}^r$: The leader credential which validates the round leader for round $r$ and can be verified by all nodes in the network.
	For example, it could be a special hash value in a Proof-of-work (PoW) protocol or the proof of possessing the chosen coin in a  Proof-of-Stake (PoS) consensus.
	In general, regardless of the consensus mechanism, credentials are linked to the public key of the leader and can be verified by a corresponding signature.
	\item $\pi{(n_i)}$: The probability of node $n_i$ being the round leader, also referred as the capacity of node $n_i$. 
	It corresponds to the mining power in PoW or the stake size in PoS protocols and is assumed to be greater than zero for every node in the network. 
	$\pi(S)$ corresponds to the total probability of the all nodes in set $S$.
	%\item $ER^T_i$: The expected reward of node $n_i$ from a transaction $T$.
	\item $\mathcal{N}_K^T$: The set of nodes who know (have) the transaction $T$. $\mathcal{N}_K^{n,T}$ presents the set from the point of view of node $n$ (including $n$ itself).
	\item $\mathcal{N}_{NK}^T$: The set of nodes who do not know (have) transaction $T$ yet. $\mathcal{N}_{NK}^{n,T}$ denotes the set from the point of view of node $n$ and includes only the neighbors of $n$.
	%\item $\mathcal{N}_K^{n,T}$: From point of view of node $n$, the set of nodes who know (have) the transaction $T$.
	%\item $\mathcal{N}_{NK}^{n,T}$: From point of view of node $n$, the set of nodes who do not know (have) transaction $T$ yet.
\end{itemize}




==> tex/LeaderSelection.tex <==
\section{Leader Selection}

Leader selection in a blockchain structure is the most crucial part regarding security, availability and efficiency. The ideal selection mechanism should provide the following properties:
\begin{itemize}
	\item At each round, leader is randomly chosen from set of participants.
	\item It tolerates failing or malicious activities of the potential leader.
	\item Each participant can easily verify validity of the leader.
\end{itemize}
Note that the first condition implicitly states that no party can gain considerable advantage to become leader in the future rounds. Recently, proposed solutions like \cite{micali2016algorand, bentovsnow, pass2016sleepy} support honest-but-lazy participants with the assumption of their presence in any necessity \todo{check}. On the other hand, selection from active participants could provide more robust and complete block construction since it is more reasonable to assume presence of the assigned leader.

%In a distributed network, leader selection is heavily correlated with joint random number generation. They both tries to randomly generate a number within a given interval, which contributed by all parties and unbiased to any malicious activities. A simple JRNG protocol can be defined as:
%\begin{enumerate}
%	\item Every participant generates a random number $r_i$ and shares its commitment $C(r_i)$.
%	\item Each participant shares his committed random number, and verifies others' commitments.
%	\item Global random number is the XOR of all commited values $R=\bigoplus_i r_i$.
%\end{enumerate}
%
%The problem with this scheme is that a malicious party can wait until he receives all $r_i$'s, then he decides to share or not his own value. This not only deviates the global random number in the favor of malicious party but also degenerates continuity of block generation. On the other hand, in a distributed network, it may cause a deadlock. In the absence of a central authority to redesign the protocol, continuity against malicious parties is a must. 
%
%In order to avoid single point of failures, blockchain mechanism should not be rely on whole participation protocols or uniquely defined leadership elections.

There are several parameters of selection protocol that causes trade-off between security and reliability of a blockchain systems.
Here, we will focus on single leader selection since transition from single selection to a subset selection can be done by simple iterations. Moreover, in most of the cases, size of the election set can be adjusted by just tuning the parameters without any additional rounds.

\subsection{Block Dependency}
Tradeoff between choosing leader from a quantity dependent or independent on the chain.\\
\textbf{Independent:}
\begin{itemize}
	\item[+] Restrict manipulation of the current leader.
	\item[-] Foresee the future leaders with some probability. 
\end{itemize}
\textbf{Dependent:}
\begin{itemize}
	\item[+] Cannot foresee the future candidates
	\item[-] Easy to manipulate
\end{itemize}

\subsection{Appearance of Quantity wrt Chain Time}
Leader selection quantity is predefined in some previous rounds, our determined during the block construction.\\
\textbf{Previous rounds:}
\begin{itemize}
	\item[+] No trials meaning no energy consumption. 
	\item[+] Easy and efficient to gather the block since the leader is known.
	\item[-] Leader may able to control the possible owners of the next round.
\end{itemize}
\textbf{Current Round:}
\begin{itemize}
	\item[+] Controlling previous rounds does not lead to any advantage.
	\item[-] Energy consumption by trials each round. 
	\item[-] Consensus on the leader is questionable, when to stop?
\end{itemize}

\subsection{Appearance of Leader in the Network wrt Chain Time}
Eligibility of being a leader may require existence in $k$ previous rounds.\\
\textbf{Previous rounds:}
\begin{itemize}
	\item[+] Eliminates last-minute manipulations
\end{itemize}
\textbf{Current Round:}
\begin{itemize}
	\item[+] Instant ability to contribute the network.
\end{itemize}

\subsection{Claiming Leadership with or without Block \todo{Is it the same with 2.2?}}
\textbf{Leader before the block creation}
\begin{itemize}
	\item[+] Efficiently gather the transactions since the end point is known
	\item[-] Failure of the leader delays progress on the chain.
\end{itemize}
\textbf{Leader simultaneously with the block}
\begin{itemize}
	\item[+] No need to worry about failure of the leader
	\item[-] Redundant work done by all miners except the leader (collecting trans.)
	\item[-] Redundant communication cost while trying to reach all miners
\end{itemize}

\subsection{Validity of Leader (Deterministic v.s. Probabilistic)}
\textbf{Deterministic:}
\begin{itemize}
	\item[+] No forking
	\item[-] May not have any candidate (like Algorand).
	\item[-] Failure of the leader even he exists
\end{itemize}
\textbf{First valid one:}
\begin{itemize}
	\item[+] No worry for appearance of the leader
	\item[-] Forks may occur even in honest cases
\end{itemize}


==> tex/Proposal.tex <==
\section{A-PoW Based Blockchain Scheme with Effective Propagation}\label{sec:a-pow}

%\subsection{Anonymous Proof-of-Work}
%In the previous section, we explained how incentive and efficient propagation mechanism can be introduced. 
%Spite of enormous bandwidth reduction, this mechanism increases block memory by including additional signatures for each transaction.
%Since there should be an evidence of each contributor to receive their shares, at least their public keys needed to be included. 
%Also, in order to prevent manipulation over a path log, signatures of nodes on the path also needed to be included.

\textit{Anonymous Proof-of-Work} (A-PoW) is proof-of-work structure which public keys of the nodes in the network are hidden in commitments and can be verified when they revealed.
Claiming the ownership without revealing identity can be done by commitment schemes. 
A-PoW is extension of the original PoW where a miner $l$ try to find a random value $R_l$ such that $H\left(H(H(R_l,PK_l)),HASH\_PREV\right)$ would be less than a predefined value $M$.
Once, he broadcasts round leader credential $\mathcal{L}^r=H(H(R_l,PK_l))$, every node can check its validity by using the hash of previous round block $HASH\_PREV$.

In recognition phase, each intermediary node convey the leader credential and path identifier.
Incoming and outgoing path identifiers of a node $n$ are denoted by $IN_{n}$ and $OUT_{n}$ which are used to validate and secure the propagation path.
Initial identifier is defined as $OUT_{l}=H(H(H(R_l,PK_l)),H(R_l,PK_l))$ and propagated to the neighbors of the round leader.
Each node $n$ chooses a random value $R_n$ and commit his public-key $PK_n$ with it, i.e., $H_n=H(R_n,PK_n)$, then updates the identifier coming from the gradient node by $OUT_{n}=H(IN_{n},H_{n})$.
This operation is done just for the gradient node (first one sending $\mathcal{L}^r$), then updated identifier and the credential are forwarded to the neighbors.
Nodes may ignore the subsequent identifiers except a client who stores the first $N_{con}$ ones for transaction phase.
Here, instead of commitments, public keys can be directly used to reduce the memory storage of each transaction, while risking exposure of the public key and network ID correlations.

After the routing paths are defined, each client delivers signed transaction and incoming identifier to his $N_{out}$ neighbors.
The first receiving nodes, check the signature, then add their commitments to the message and forward it to their gradient nodes.
From that point, each intermediary node $n$ in the path, first checks the validity of the path via the commitments included and their own identifiers, then forward the message including their commitments to the gradient node.

Once transactions are received by the round leader, he includes the ones which are valid in transaction manners as well as the propagation path structure.
The block consists of the credential, hash of previous block ($HASH\_PREV$), valid transactions, committed values $PK_l$ and $R_l$ and signature of the block.
Then, the block is propagated through the network.

%At the end, by opening the proof and adding to the block, it can be validated. 

%A-PoW consensus mechanism can be deployed in case where the incentive for propagation is not required but DDoS-like attacks are taken into account.

%A round of the A-PoW blockchain is functioning as follows: 
%\begin{enumerate}
%	\item \textit{Recognition phase}: A potential leader node $n_k$ claim leadership via A-PoW including $H(rand_k,Sign(rand_k))$, $L^r\equiv\text{A-PoW}$ is propagated.
%	\item \textit{Transaction phase}: All transactions are propagated signed by the intermediary nodes.
%	\item The potential leader $n_k$ broadcast the block $B^r$ including commitment $rand_k$ and all transactions.
%\end{enumerate}

\alglanguage{pseudocode}
\begin{algorithm}[H]
\begin{algorithmic}
%\Require Leader credential $\mathcal{L}^r$
%\Ensure For each node, closest node to the leader $cn_i$, for $i=1,\ldots,n$
\State
\State \underline{A-PoW}
\State A miner $l$ finds a random $R_l$ value such that
\State \quad $H\left(H(H(R_l,PK_l)),HASH\_PREV\right)<M$
\State
\State \underline{Recognition Phase}
\State Leader $l$ propagates $\mathcal{L}^r=H(H(R_l,PK_l))$ and $OUT_0=H(\mathcal{L}^r,H(R_l,PK_l))$.
\For{Each node $n_i$}
\If{First time receiving $\mathcal{L}^r$ and $IN_{n'}$}
\If{$H\left(\mathcal{L}^r,HASH\_PREV\right) \stackrel{?}{<} M$}
\State Assign $IN_{n_i}\leftarrow IN_{n'}$ and gradient node as $n'$
\State Compute $OUT_{n_i}=H(IN_{n_i},H_{n_i})$, where $H_{n_i}=H(R_{n_i},PK_{n_i})$
\State Propagate $\mathcal{L}^r$ and $OUT_{n_i}$ to neighbors.
\EndIf
%\If{Client of $c_T$}
%\State Store the first $N_{out}$ incoming $IN$ values
%\EndIf
\EndIf
\EndFor
\State 
\State \underline{Transaction Phase}
\State  Client provides $Signed(T,IN_{c_T})$ (and $\mathcal{H}=\emptyset$) to the first $N_{out}$ gradient nodes.
\For{Each node $n_i$ receiving $Signed(T,IN_{c_T})$ and $\mathcal{H}$}
\If{First time receiving $T$}
\If{Signature path holds}
\State Update $\mathcal{H}\leftarrow \mathcal{H} \bigcup \{ H_{n_i} \}$
\State Send $Signed(T,IN_{c_T})$ and $\mathcal{H}$ to the gradient node.
\EndIf
\EndIf
\EndFor
\end{algorithmic}
\caption{A round of A-PoW protocol} 
\label{alg:a-pow}
\end{algorithm}

\begin{figure}
	\begin{center}
		\includegraphics[width=\textwidth]{figures/a-pow.pdf}
		\caption{Illustration of a path between the round leader and a client in A-PoW. Upper-side and solid arrows represent the recognition phase while the lower side and dashed arrows do the transaction phase.}
	\end{center}
\end{figure}

\paragraph{Privacy and Memory Trade-off.}
In almost all blockchain schemes, since there is no incentive for propagation, there is no reason to keep track of propagation path.
Previous works having incentive utilize signature chains where each node signs the message and the public key of receiver.
Signature chains cause direct connection between nodes network ID and their public keys.
In addition, they have to store signatures of all contributing nodes along with their public keys.

This scheme enables to use the same network structure without compromising the identities of the nodes except clients and round leaders. The location of round leader and clients will be known to their neighbors, and they may need to update their key pairs or replace their connections.
The path is stored like a binary tree, and each contributor can demand his fee by proof of his public key and random value matching with his commitment.
Irrelevant parties may just store the root of the tree.
In addition, if the network and public key correlations is brushed off, then public keys can be directly used instead of commitments.
This would result in nearly optimal storage burden since storage of public keys is necessary for payments.

%\paragraph{Privacy.}
%Thus, A-PoW consensus protocol has the same security level as any first-leader-then-block scheme against DDoS, impersonation and corruption attacks.
%With routing mechanism and A-PoW, we can enjoy the same security as in Bitcoin with much less bandwidth usage.

\paragraph{Incentive for Block Propagation.}
As a consequence of the routing and incentive mechanisms, intermediary nodes also have incentive to propagate the block since they share transaction fees. 
Even, the ones who are closer to the leader would have more motivation since they probably gain from more transactions.
%Therefore, it encourages even more to share rather than selfish mining.

%\paragraph{\todo{Microblock Case.}}
%We refer Bitcoin-NG for microblocks type implementation where the leader is validated by the PoW in key block, then he propose several microblocks including only transactions.
%In A-PoW, microblocks can be validated by  
%
%\todo{For one block, include PK and signed whole block with SK.
%For multiple case, $H_0 < H^i(H_0)$, for each microblock include HASH\_PREV and $H^2k-i(H_0)$.
%Only the last one can be manipulated.
%In this way, Pk of round leader is never revealed.}
